Sim-to-Real Transfer of Robotic Assembly with Visual Inputs Using CycleGAN and Force Control

Recently, deep reinforcement learning (RL) has shown some impressive successes in robotic manipulation applications. However, training robots in the real world is nontrivial owing to sample efficiency and safety concerns. Sim-to-real transfer is proposed to address the aforementioned concerns but introduces a new issue called the reality gap. In this work, we introduce a sim-to-real learning framework for vision-based assembly tasks and perform training in a simulated environment by employing inputs from a single camera to address the aforementioned issues. We present a domain adaptation method based on cycle-consistent generative adversarial networks (CycleGAN) and a force control transfer approach to bridge the reality gap. We demonstrate that the proposed framework trained in a simulated environment can be successfully transferred to a real peg-in-hole setup.

==> tables/ffheva_influence_success_400.tex <==
% bath detergent + 20%. was 30%, 94 pos, 226 neg
%\vspace*{2mm}
\begin{table}[!h]
    \vspace*{0.5em}
    % \begin{adjustwidth*}{}{-\marginparwidth-\marginparsep}
    \caption{FFHEVALUATOR INFLUENCE ON GRASPING SUCCESS}
    \centering
    \resizebox{\columnwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|}
        \hline
        \textbf{Object}     & \textbf{Th=0.0} & \textbf{Th=0.5} & \textbf{Th=0.7} & \textbf{Th=0.9} & \textbf{Th=0.95} \\
        \hline
        BakingSoda          & 75\%            & 86\%            & 88\%            & 97\%            & -                \\
        BathDetergent       & 51\%            & 57\%            & 70\%            & 86\%            & 83\%             \\
        BroccoliSoup        & 82\%            & 82\%            & 90\%            & 82\%            & -                \\
        CoughDrops     & 73\%            & 72\%            & 77\%            & 89\%            & 99\%             \\
        Curry               & 56\%            & 73\%            & 80\%            & 90\%            & 94\%             \\
        FizzyTablets & 43\%            & 63\%            & 77\%            & 89\%            & 85\%             \\
        InstantSauce        & 64\%            & 72\%            & 74\%            & 72\%            & 92\%             \\
        NutCandy            & 56\%            & 65\%            & 70\%            & 74\%            & -                \\
        PotatoeDump.    & 70\%            & 77\%            & 93\%            & 80\%            & 90\%             \\
        Sprayflask          & 52\%            & 53\%            & 80\%            & 91\%            & 92\%             \\
        TomatoSoup          & 63\%            & 64\%            & 66\%            & 70\%            & 99\%             \\
        YellowCube     & 48\%            & 60\%            & 64\%            & 69\%            & 85\%             \\
        \hhline{|=|=|=|=|=|=|}
        Avg. Success     & 61\%            & 70\%            & 75\%            & 82\%            & 91\%             \\
        \hline
        Coverage            & 99\%            & 87\%            & 83\%            & 28\%            & 5\%              \\
        \hline
    \end{tabular}}
    % \vspace{-1em}
    \label{table:ffheva_influence_success}
\end{table}

==> tables/run_time.tex <==
% bath detergent + 20%. was 30%, 94 pos, 226 neg

\begin{table}[!h]
    \centering
    \caption{RUNTIME COMPARISON WITH OTHER METHODS}
    \setlength{\tabcolsep}{8pt}
    \begin{tabular}{cc@{\hspace{0.6\tabcolsep}}cc}
        \hline
        \textbf{Authors} & \textbf{Methods}    & \textbf{Success Rate} & \textbf{Time}\\
        \hline
        Liu et al. \cite{liu2019generating}  & direct regression   & 80.0\%                 & 3-5s   \\
        Lu et al. \cite{lu2020multifingered}   & gradient-based opt. &75.0\%       & 5-10s            \\
        Lundell et al. \cite{lundell2020multi} & GAN-based & 60.0\%      & 9.1s              \\ 
        Kiatos et al. \cite{Kiatos2021Sampling} &  shape completion &86.3\%      & 4.25s           \\
        Ours & FFHNet (cVAE)    & \textbf{91.0\%}    & \textbf{30ms}    \\

        \hline
    \end{tabular}
    %\caption{}
    \vspace{-1em}
    \label{table:runtime}
\end{table}

==> tables/success_compare.tex <==
% bath detergent + 20%. was 30%, 94 pos, 226 neg

\begin{table}[!h]
    \centering
    \caption{PERFORMANCE COMPARISON}
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{|c@{\hspace{1\tabcolsep}}|c|c|c|}
        \hline
        Method & \textbf{\thead{Heuristics-based\\ (Sec. \ref{sec:data_generation}) }}     & \textbf{FFHGenerator} & \textbf{\thead{FFHGenerator +\\ FFHEvaluator}}\\
        \hline
        Success & 15\% & 61\% & \textbf{91\%} \\

        \hline
    \end{tabular}
    %\caption{}
    \vspace{-1em}
    \label{table:success_rate}
\end{table}
